Continuous Transfer Learning for UAV Communication-aware Trajectory Design

Deep Reinforcement Learning (DRL) emerges as a prime solution for Unmanned Aerial Vehicle (UAV) trajectory planning, offering proficiency in navigating high-dimensional spaces, adaptability to dynamic environments, and making sequential decisions based on real-time feedback. Despite these advantages, the use of DRL for UAV trajectory planning requires significant retraining when the UAV is confronted with a new environment, resulting in wasted resources and time. Therefore, it is essential to develop techniques that can reduce the overhead of retraining DRL models, enabling them to adapt to constantly changing environments. This paper presents a novel method to reduce the need for extensive retraining using a double deep Q network (DDQN) model as a pretrained base, which is subsequently adapted to different urban environments through Continuous Transfer Learning (CTL). Our method involves transferring the learned model weights and adapting the learning parameters, including the learning and exploration rates, to suit each new environment specific characteristics. The effectiveness of our approach is validated in three scenarios, each with different levels of similarity. CTL significantly improves learning speed and success rates compared to DDQN models initiated from scratch. For similar environments, Transfer Learning (TL) improved stability, accelerated convergence by 65%, and facilitated 35% faster adaptation in dissimilar settings.

==> name.tex <==
\section*{Problem Formulation}

\subsection*{Objective}
Optimize the UAV's trajectory to minimize the weighted sum of the mission completion time and the expected communication outage duration, leveraging previous experience through Transfer Learning.

\subsection*{Parameters}
\begin{itemize}
    \item $R$: Radio map indicating communication strengths at various locations.
    \item $S$: Set of states representing possible locations of the UAV.
    \item $A$: Set of actions representing possible trajectories or moves of the UAV.
    \item $T(s, a)$: Expected time to complete the mission when moving from state $s$ following action $a$.
    \item $O(s, a, R)$: Expected communication outage duration when moving from state $s$ following action $a$ based on the radio map $R$.
    \item $E(s, a)$: Energy consumed by the UAV when moving from state $s$ following action $a$.
    \item $M$: Maximum allowed energy consumption.
\end{itemize}


\begin{itemize}
    \item $G$: Geographical area under consideration divided into grid points.
    \item $T$: Set of base stations or transmitters in the area.
    \item $P_t$: Power transmitted by a base station $t \in T$.
    \item $L_{gt}$: Path loss between grid point $g$ and transmitter $t$.
    \item $N_g$: Noise level at grid point $g$.
\end{itemize}


\begin{itemize}
    \item $R_g$: Received signal strength (RSS) at grid point $g \in G$.
\end{itemize}

\subsection*{Signal Model}
For each grid point in the geographical area, the RSS can be modeled as:
\begin{equation}
    R_g = P_t - L_{gt} + N_g \quad \forall g \in G, \forall t \in T
\end{equation}

\subsection*{Path Loss Model}
The path loss can be modeled using various methods. A common model is the log-distance path loss model:
\begin{equation}
    L_{gt} = L_0 + 10 \alpha \log_{10}\left(\frac{d_{gt}}{d_0}\right)
\end{equation} 
Where:
\begin{itemize}
    \item $L_0$ is the path loss at a reference distance \(d_0\).
    \item \(d_{gt}\) is the distance between grid point \(g\) and transmitter \(t\).
    \item \(\alpha\) is the path loss exponent.
\end{itemize}

\subsection*{Noise Model}
Noise can be considered as a Gaussian variable with zero mean and variance \(\sigma^2\). However, for a deterministic map, we can take the average noise level:
\begin{equation}
    N_g = \sigma^2 \quad \forall g \in G
\end{equation}

\subsection*{Final Radio Map}
Using the above models, a radio map can be generated which provides the RSS value at each grid point, taking into account the power from all transmitters, path loss, and noise.

\subsection*{Decision Variables}
\begin{itemize}
    \item $Q(s, a; \bm{\theta})$: Approximated Q-value represented by a neural network with parameters $\bm{\theta}$, where the input is state $s$ and action $a$, and the output is the Q-value.
\end{itemize}         

\subsection*{Objective Function}
Minimize the weighted sum of mission completion time, expected communication outage duration, and energy consumption:
\begin{equation}
    \min_{a \in A} \sum_{s \in S} \left( \omega_1 T(s, a) + \omega_2 O(s, a, R) + \omega_3 E(s, a) \right)
\end{equation}
Where:

\begin{itemize}
    \item $\omega_1, \omega_2,$ and $\omega_3$ are weighting factors balancing mission completion time, outage duration, and energy consumption, respectively.
\end{itemize}


\subsection*{Constraints}
\begin{equation}
    \sum_{s \in S} E(s, a) \leq M \quad \forall a \in A
\end{equation}
